Evaluating Metrics for Bias in Word Embeddings

Over the last years, word and sentence embeddings have established as text preprocessing for all kinds of NLP tasks and improved the performances significantly. Unfortunately, it has also been shown that these embeddings inherit various kinds of biases from the training data and thereby pass on biases present in society to NLP solutions. Many papers attempted to quantify bias in word or sentence embeddings to evaluate debiasing methods or compare different embedding models, usually with cosine-based metrics. However, lately some works have raised doubts about these metrics showing that even though such metrics report low biases, other tests still show biases. In fact, there is a great variety of bias metrics or tests proposed in the literature without any consensus on the optimal solutions. Yet we lack works that evaluate bias metrics on a theoretical level or elaborate the advantages and disadvantages of different bias metrics. In this work, we will explore different cosine based bias metrics. We formalize a bias definition based on the ideas from previous works and derive conditions for bias metrics. Furthermore, we thoroughly investigate the existing cosine-based metrics and their limitations to show why these metrics can fail to report biases in some cases. Finally, we propose a new metric, SAME, to address the shortcomings of existing metrics and mathematically prove that SAME behaves appropriately.

==> extras.tex <==


% Further formalizations
\begin{comment}
\subsection{Further Formalization} % TODO besserer titel

In this section, we will introduce further definitions that will be relevant for later proofs. If not stated otherwise, we will consider 'words' as word vectors $\bm{w} \in V$. We define bias in terms of a concept $A = \{A_1, ..., A_n\}$ distinguishing between $n \geq 2$ groups, represented by a list of attribute sets $A_i = \{a_{i1}, ..., a_{im}\}$ with attributes $a_{ik} \in V$. Regarding these attribute sets, we make the following definitions: \\

\begin{definition}
	\label{def:attr_set_center}
	The center of an attribute set $A_i$ is given by $\bm{a_i^*} = \frac{1}{m} \sum_{k = 0}^{m} a_{ik}$. %normalize?
\end{definition}


\begin{definition}
	\label{def:attr_set_diff}
	Two attribute sets $A_i, A_j$ are different if $a_i^* \neq a_j^*$.\\
\end{definition}

\begin{definition}
	\label{def:bias_comparablity}
	Attribute sets $A_i$, $A_j$ are pairwise comparable, if $|A_i| = |A_j|$ and for any attribute $a_{ik} \in A_i$ there is an attribute $a_{jk} \in A_j, a_{jk} \neq a_{ik}$ with the (semantic and syntactic) meanings of $a_{ik}$ and $a_{jk}$ only differing by their group membership. The attributes $a_{ik}$ and $a_{jk}$ are also called pairwise comparable.\\
	We call all attribute sets $A = \{A_1, ..., A_n\}$ comparable if any pair $A_i, A_j \; i, j \in \{1..n\}, i\neq j$ is pairwise comparable, and similarly $\{a_{ik}\}_{i \in {1..n}}$ comparable if any pair $a_{ik}, a_{jk} \; i, j \in \{1..n\}, i\neq j$ is pairwise comparable.
\end{definition}

Given a comparable concept $A$, we can determine a bias subspace $B \subset V$ and neutral subspace $N \subset V$ with $B$ describing all relation between the attribute sets in $A$ (similarly to \cite{NIPS2016_a486cd07}):
\begin{definition}
	\label{def:bias_subspace}
	The bias subspace $B \subset V$ regarding a comparable concept $A$ is the smallest possible subspace describing the relations between all comparable attributes $a_{ik}$ and $a_{jk}$, i.e. $(a_{ik} - a_{jk}) \in B \; \forall \; i, j \in {1..n}, i\neq j$.
\end{definition}
\begin{definition}
	\label{def:neutral_subspace}
	The neutral subspace $N \subset V$ regarding a comparable concept $A$ is the complementary subspace to the bias subspace, i.e. $B \cap N = \{0\}$ and $B + N = V$.
\end{definition}
%In the following, we assume the bias concept $A$ to be comparable. Thus, any word $\bm{w}$ can be described by a linear combination of vectors in $B$ and $N$: $\bm{w} = b\bm{w_b} + (1-b)\bm{w_n}, \; \bm{w_n} \in N, \bm{w_b} \in B, |\bm{w_b}| = |\bm{w_n}| = 1, 0 \leq b \leq 1$. Then $b$ determines the bias of word $\bm{w}$. Intuitively, for $b = 1$ the words would be maximally biased, since it's defined solely in the bias subspace, for $b = 0$ it would be fair, since it has no bias component. This reflects the idea behind Bolukbasi's debiasing method \cite{NIPS2016_a486cd07}.\\

Since any word $\bm{w} = b\bm{w_b} + (1-b)\bm{w_n}$ with $b > 0$ can not be equidistant to all attributes that define the bias subspace, it is possible to calculate the bias using the distances between $\bm{w}$ and the different attributes. Accordingly, the cosine seimiliary is used as a proximity measure.

For consistent attribute sets $A_i$ we can simplify equation \eqref{eq:attr_sim} to \begin{eqnarray}
\label{eq:attr_sim_center}
s(\bm{w},A_i) &=& cos(\bm{w}, \bm{a_i*}).
\end{eqnarray}
Based on this, we consider a word $\bm{w}$ biased in favor of $A_i$ compared to $A_j$ if
\begin{eqnarray}
\label{eq:compare_attr}
&&s(\bm{w},A_i) > s(\bm{w}, A_j)\\
&\iff& cos(\bm{w}, \bm{a_i*}) > cos(\bm{w}, \bm{a_j*})
\end{eqnarray}
and $A_i$ the attribute that $\bm{w}$ is maximally biased towards (both negative + positive) if 
\begin{eqnarray}
\label{eq:closest_attr}
&&s(|\bm{w},A_i)| > |s(\bm{w}, A_j)| \; \forall \; A_j \in A, j \neq i \\
&\iff& |cos(\bm{w}, \bm{a_i*})| > |cos(\bm{w}, \bm{a_j*})| \; \forall \; A_j \in A, j \neq i.
\end{eqnarray}

\end{comment}





% WEAT magntiude comparable Lemma + Theorem für 4 Beispielwörter
\begin{lemma} \label{theor:schranke1}
Let $x_1,x_2,x_3,x_4 \in \R$ be real numbers. Let
$\hat{\mu},\hat{\sigma}$ denote the empirical estimate of mean and
standard deviation of $x_i$. Then, for $i \neq j$, the following bound holds
\begin{align*}
    \left| \frac{x_i - \hat{\mu}}{\hat{\sigma}} + \frac{x_j -
\hat{\mu}}{\hat{\sigma}} \right| \leq 2.
\end{align*}
Furthermore, the bound is obtained if and only if $x_i = x_j = -x_k =
-x_l$ for $\{k,l,i,j\} = \{1,2,3,4\}$.
\begin{proof}
\newcommand{\x}{\mathbf{x}}
Let $f(x) = ax+b$ be a linear function. Then the images of $x_i$ under
$f$ have mean $a\hat{\mu}+b$ and standard deviation $|a|\hat{\sigma}$.
On the other hand, we have
\begin{align*}
    \frac{f(x_i)-(a\hat{\mu}+b)}{a\hat{\sigma}}
    &= \frac{(ax_i+b)-(a\hat{\mu}+b)}{a\hat{\sigma}}
    \\&= \frac{x_i-\hat{\mu}}{\hat{\sigma}}.
\end{align*}
Thus, applying $f$ does not change the bound and therefore we may reduce
to case of $\hat{\mu} = 0$ and $\hat{\sigma} = 1$. This allows us to
rephrase the problem of finding the maximal bound as an optimization
problem:
\begin{align*}
    \min \quad& (1,1,0,0) \cdot \x \\
    \text{s.t.} \quad & \x^\top I \x = 4\\
                      & \mathbf{1}^\top \x = 0,
\end{align*}
where $\x = (x_1,x_2,x_3,x_4)^\top$, $I$ is the identity matrix and
$\mathbf{1}$ denotes the vector consisting of ones only. Notice, that we
assumed w.l.o.g. that $i,j = 1,2$. Furthermore, we made use of the
symmetry properties to replace $\max |(1,1,0,0)^\top \x|$ by the
minimizing statement above, $\hat{\mu} = 0$ is expressed by the last and
$\hat{\sigma} = 1$ by the first constraint (recall that $\hat{\sigma}
=  \sqrt{1/4 \x^\top \x-\hat{\mu}^2}$).

It is easy to see that $\x^* = (-1,-1,1,1)^\top$ fulfills the
constraints and lies within the stated bound. We will now proceed by
showing that it is a global optimum. As can be seen the problem stated
above is a QCQP, thus, if we relax the first constraint to $\x^\top I
\x \leq 4$ we obtain a convex problem. It follows that it suffices to
show that $\x^*$ is a local optimum:
The Lagrangien of the problem above and its first two derivatives are
given by
\begin{align*}
    L(\x,\lambda_1,\lambda_2) &= (1,1,0,0) \cdot \x - \lambda_1 (\x^\top
I \x - 4) - \lambda_2 \mathbf{1}^\top \x \\
    \nabla_x L(\x,\lambda_1,\lambda_2) &= (1,1,0,0)^\top - 2 \lambda_1
\x - \lambda_2 \mathbf{1} \\
    \nabla^2_{x,x} L(\x,\lambda_1,\lambda_2) &= - 2 \lambda_1 I.
\end{align*}
To assure $\nabla_x L(\x^*,\lambda_1^*,\lambda_2^*) = 0$ we have to set
$\lambda_1^* = -1/4$ and $\lambda_2^* = 1/2$, which fulfills the
necessarily KKT conditions for both the original and the convex problem.
Now, as $\nabla^2_{x,x} L(\x^*,\lambda_1^*,\lambda_2^*) = 1/2 I$ is
positive definite, we see that $\x^*$ is a global optimum, indeed.

Furthermore, we can write $\nabla_x L(\x,\lambda_1,\lambda_2) = 0$ as
the following linear equation system:
\begin{align*}
    \begin{bmatrix} 2x_1 & 1 \\ 2x_2 & 1 \\ 2x_3 & 1 \\ 2x_4 & 1
\end{bmatrix} \begin{bmatrix} \lambda_1 \\ \lambda_2 \end{bmatrix} &=
\begin{bmatrix} 1 \\ 1 \\ 0 \\ 0 \end{bmatrix}.
\end{align*}
Subtracting the first from the second and the third from the fourth row
we see that $2(x_2-x_1)\lambda_1 = 0$ and $2(x_4-x_3)\lambda_1 = 0$,
which either implies $\lambda_1 = 0$ or $x_1=x_2$ and $x_3=x_4$.
However, assuming $\lambda_1 = 0$ would imply that $\lambda_2 = 1$ from
the first or second row and $\lambda_2 = 0$ from the third or fourth
row, which is a contradiction. Thus, we have  $x_1=x_2$ and $x_3=x_4$.
But the second constraint from the optimization problem can then only be
fulfilled if $2x_1+2x_3 = 0$ and this implies $x_1 = -x_3$. In this case
the first constraint is equal to $4x_1^2 = 4$. So $\x^*$ and $-\x^*$
where the only KKT points to begin with.
The statement follows.
\end{proof}
\end{lemma} 




\begin{theorem}
The effect size $d(X,Y,A,B)$ of WEAT with $X=\{\vec{x}_1,\vec{x}_2\}, Y=\{\vec{y}_1,\vec{y}_2\}$ is \extremaVgl.

\begin{proof}
With $c_i = s(\vec{x_i},A,B)$, $c_{i+2} = s(\vec{y_i},A,B)$, $\hat{\mu}=0.25 \sum^4_i c_i$ and $\hat{\sigma}=\sqrt{0.25\sum^4_i (c_i - \mu)^2}$, we have
\begin{align}
    d &= \frac{0.5(c_1 + c_2) - 0.5(c_3 + c_4)}{\hat{\sigma}} \\
      &= \frac{0.5(c_1- \hat{\mu} + c_2 - \hat{\mu}) - 0.5(c_3 - \hat{\mu} + c_4 - \hat{\mu})}{\hat{\sigma}} \nonumber \\
      &= \frac{(c_1- \hat{\mu}) + (c_2 - \hat{\mu}) - (c_3 - \hat{\mu}) - (c_4 - \hat{\mu})}{2\hat{\sigma}} \nonumber \\
      &= \frac{2(c_1- \hat{\mu}) + 2(c_2 - \hat{\mu}) - \sum^4_i(c_i - \hat{\mu})}{2\hat{\sigma}} \nonumber \\
      &= \frac{(c_1- \hat{\mu}) + (c_2 - \hat{\mu})}{\hat{\sigma}} \in [-2,2],
\end{align}
where the last statement follows from Lemma \ref{theor:schranke1}. The extreme value $\pm 2$ is reached if $c_1=c_2=-c_3=-c_4$, which can be obtained by setting $\vec{x}_1=\vec{x}_2=-\vec{y}_1=-\vec{y}_2$, independently of $A$ and $B$ as long as $A \neq B$ and $\sum_{\vec{a}_i \in A} \vec{a}_i/\|\vec{a}_i\| \neq 0 \neq \sum_{\vec{b}_i \in B} \vec{b}_i/\|\vec{b}_i\|$.
\end{proof}
\end{theorem} 
